Accurate Weakly-Supervised Deep Lesion Segmentation using Large-Scale Clinical Annotations: Slice-Propagated 3D Mask Generation from 2D RECIST

Volumetric lesion segmentation from computed tomography (CT) images is a powerful means to precisely assess multiple time-point lesion/tumor changes. However, because manual 3D segmentation is prohibitively time consuming, current practices rely on an imprecise surrogate called response evaluation criteria in solid tumors (RECIST). Despite their coarseness, RECIST markers are commonly found in current hospital picture and archiving systems (PACS), meaning they can provide a potentially powerful, yet extraordinarily challenging, source of weak supervision for full 3D segmentation. Toward this end, we introduce a convolutional neural network (CNN) based weakly supervised slice-propagated segmentation (WSSS) method to 1) generate the initial lesion segmentation on the axial RECIST-slice; 2) learn the data distribution on RECIST-slices; 3) extrapolate to segment the whole lesion slice by slice to finally obtain a volumetric segmentation. To validate the proposed method, we first test its performance on a fully annotated lymph node dataset, where WSSS performs comparably to its fully supervised counterparts. We then test on a comprehensive lesion dataset with 32,735 RECIST marks, where we report a mean Dice score of 92% on RECIST-marked slices and 76% on the entire 3D volumes.

==> data/side_by_side.tex <==
% !TEX root = ../DeepLesion.tex
\begin{table}[t]
\centering
\caption{Table}
\label{tab:side-by-side}
\makebox{%
	\begin{minipage}[b]{0.49\linewidth}
	\centering
	\subcaptionbox{Mask init.} 
	{\scriptsize
	\begin{tabular}{l c c c}
		\hline
		Method & Recall & Precision & mDICE \\ \hline
		\multicolumn{4}{c}{Lymph Node} \\ \hline
		RECIST     & 0.35$\pm$0.09  & \textBF{0.99$\pm$0.05}  & 0.51$\pm$0.09 \\
		DCRF      & 0.29$\pm$0.20  & 0.98$\pm$0.05  & 0.41$\pm$0.21 \\
		GrabCut    & 0.10$\pm$0.25  & 0.32$\pm$0.37  & 0.11$\pm$0.26 \\
		GrabCut$^i$& 0.53$\pm$0.24  & 0.92$\pm$0.10  & 0.63$\pm$0.17 \\
		GrabCut-R  & \textBF{0.83$\pm$0.11}  & 0.86$\pm$0.11  & \textBF{0.83$\pm$0.06} \\ \hline
		\multicolumn{4}{c}{Deep Lesion RECIST-Slice (Testing Images)} \\ \hline
		RECIST     & 0.39$\pm$0.13  & \textBF{0.92$\pm$0.14}  & 0.53$\pm$0.14 \\
		DCRF      & 0.72$\pm$0.26  & 0.90$\pm$0.15  & 0.77$\pm$0.20 \\
		GrabCut    & 0.62$\pm$0.46  & 0.68$\pm$0.44  & 0.62$\pm$0.46 \\
		GrabCut$^i$& \textBF{0.94$\pm$0.11}  & 0.81$\pm$0.16  & 0.86$\pm$0.11 \\
		GrabCut-R  & \textBF{0.94$\pm$0.10}  & 0.89$\pm$0.10  & \textBF{0.91$\pm$0.08} \\
		\hline
	\end{tabular}
	}
	\end{minipage}
    \hfill
    \begin{minipage}[b]{0.49\linewidth}
    \centering
	\subcaptionbox{2D conv.}
	{\scriptsize
	\begin{tabular}{l c c } %c|}
		\hline
		Method & CNN & CNN-GC \\ \hline
		\multicolumn{3}{c}{Lymph-Node} \\ \hline
		Full-Sup (HNN) & \textBF{0.710$\pm$0.18} & \textBF{0.845$\pm$0.06}  \\
		RECIST         & 0.614$\pm$0.17 & 0.844$\pm$0.06 \\
		GC-Mask        & 0.702$\pm$0.17 & 0.844$\pm$0.06  \\
		\hline
		\multicolumn{3}{c}{Deep-Lesion RECIST-Slice} \\ \hline
		Full-Sup (UNet)& 0.728$\pm$0.18 & 0.838$\pm$0.16  \\
		Full-Sup (HNN) & 0.837$\pm$0.16 & 0.909$\pm$0.10  \\
		RECIST         & 0.644$\pm$0.14 & 0.801$\pm$0.12  \\
		GC-Mask        & \textBF{0.906$\pm$0.09} & \textBF{0.915$\pm$0.10}  \\
		\hline
	\end{tabular}
	}
    \end{minipage}
}
\end{table}


==> figures/recist.tex <==
%!TEX root=../DeepLesion.tex
\begin{wrapfigure}{r}{3cm}
	% trim={<left> <lower> <right> <upper>}
	\includegraphics[width=\linewidth,page=2,trim={0cm 7cm 22.5cm 0cm}, clip]{./figures/Figures.pdf}
\end{wrapfigure} 
